Collective biological computation of metabolic economy

Presented with sensory challenges, living cells employ extensive noisy, fluctuating signalling and communication among themselves to compute a physiologically proper response which often results in symmetry breaking. We propose, based on the results of a coupled stochastics oscillators model that biological computation mechanism undertaken by insulin secreting beta-cells consists of a combination of dual intracellular Ca$^{2+}$ release processes to ensure multilayered exploration contributing to enhanced robustness and sensitivity. The computational output is what is macroscopically observed as disorder-order phase transition in collective beta-cell response to nutrient concentration increase. Based on the analogies from previoulsy described examples of biological computation, we argue that the initial response may be followed by an adaptive phase to expand the sensory spectrum and consolidate memory.

==> lte.tex <==
Prof. Dr. Jessica Flack
Santa Fe Institute, 1399 Hyde Park Road, Santa Fe, NM 87501, USA

Prof. Dr. David Wolpert
Santa Fe Institute, 1399 Hyde Park Road, Santa Fe, NM 87501, USA



Maribor and Vienna, 15.6.2022

Dear Professor Flack, Dear Professor Wolpert, 

we are submitting our manuscript "Collective biological computation of metabolic economy" to the Special Issue "Foundations of Biological Computation" of the journal Entropy. In our paper we are addressing biological computation of insuling secreting beta-cells and their collective agency through which they must timely and precisely respond to organisms metabolical needs. We have shown, using a model of coupled stochastic oscillators, that such physiological process is an example of biological computation consisting of a combination of dual intracellular calcium release processes where the crucial computational step is performed by swithcing between two modes to ensurte precise and adaptive sensing. The output of this collective biological computation is on macroscopic level empirically observed as symmetry breaking in disorder-order phase transition. 

We believe that our paper will be a valuable contribution to this excellent and exciting challenge on foundations of biological computation.


Sincerely, 
Dean Korošak,
Andraž Stožer,
Marjan Slak Rupnik
